Towards a Human-like Open-Domain Chatbot

We present Meena, a multi-turn open-domain chatbot trained end-to-end on data mined and filtered from public domain social media conversations. This 2.6B parameter neural network is simply trained to minimize perplexity of the next token. We also propose a human evaluation metric called Sensibleness and Specificity Average (SSA), which captures key elements of a human-like multi-turn conversation. Our experiments show strong correlation between perplexity and SSA. The fact that the best perplexity end-to-end trained Meena scores high on SSA (72% on multi-turn evaluation) suggests that a human-level SSA of 86% is potentially within reach if we can better optimize perplexity. Additionally, the full version of Meena (with a filtering mechanism and tuned decoding) scores 79% SSA, 23% higher in absolute SSA than the existing chatbots we evaluated.

==> Towards a Human-like Open-Domain Chatbot/advance_ssa.tex <==
In this section we take the interactive SSA from $72\% \pm 1\%$, for \meenabase{}, to $79\% \pm 1\%$, for \meenafull{}, by further tuning our decoding strategy and adding a rule to detect cross turn repetitions.

\subsection{Advancing Decoding}

We evaluate both temperature $T$ and top-\textit{k} to mitigate negative effects from the tail of the distribution \citep{holtzman19}. We chose top-\textit{k} (\textit{k} = 40) and $T=1.0$ following \citet{fan18, gpt2, keskar19, ippolito19b}. With this setting and maintaining $N=20$, we note an SSA increase from 72\% to 74\% relative to sampling from the whole vocabulary with $T=0.88$. This result is the same for both the interactive and the static evaluation.

We also swept the number of samples in sample-and-rank, evaluating $N \in \{1, 20, 400\}$. The results show that $N=20$ provides a significant improvement over $N=1$, with an absolute improvement in SSA of ${\sim}10\%$ (Figure \ref{fig:decoding-ssa}). However, $N=400$ demonstrates worse performance for sensibleness (Figure \ref{fig:decoding-sensibleness} in the appendix) and diminishing returns over $N=20$ for specificity (Figure \ref{fig:decoding-specificity} in the appendix). The significant improvement from sample-and-rank with $N=20$ motivates future work exploring alternate ranking functions and tuning parameters.

\begin{figure}[ht!]
\centering
\includegraphics[width=230pt]{fig/decoding-ssa.pdf}
\caption{Static SSA over number of sampled responses for top-\textit{k} and sampling with temperature.}
\label{fig:decoding-ssa}
\end{figure}

\subsection{Addressing Cross-turn Repetitions}

In interactive evaluation, about one third of the conversations with \meenabase{} contain cross-turn repetitions toward the end. Cross-turn repetition means that one turn somewhat repeats an earlier turn. For illustration, we cherry picked particularly problematic examples of cross-turn repetition shown in Tables \ref{t:rep1} and \ref{t:rep2}.

\begin{table}
\small
\centering
\begin{tabular}{rp{6cm}}
\toprule
\multicolumn{2}{c}{{\bf Cross-turn Repetition Example 1}} \\
\midrule
\textbf{Human}: & \textit{Hi!} \\
\textbf{Meena}: & \textit{Hi! How are you?! :)} \\
\textbf{Human}: & \textit{doing good, what would be the best city to visit in Europe?} \\
\textbf{Meena}: & \textit{Paris, Barcelona, Amsterdam, Prague} \\
\textbf{Human}: & \textit{great list! why?} \\
\textbf{Meena}: & \textit{Paris is a beautiful city, and Barcelona is too. And I've always wanted to go to Amsterdam and Prague and have never been.} \\
\textbf{Human}: & \textit{have you even been to India?} \\
\textbf{Meena}: & \textit{No, but I'd love to go.} \\
\textbf{Human}: & \textit{how about Japan?} \\
\textbf{Meena}: & \textit{I'd love to go to Japan too.} \\
\textbf{Human}: & \textit{how about Paris?} \\
\textbf{Meena}: & \textit{I'd love to go to Paris too.} \\
\textbf{Human}: & \textit{are you lying to me?} \\
\textbf{Meena}: & \textit{I'd love to go to Japan too.} \\
\textbf{Human}: & \textit{i think you're lying to me, that makes me sad} \\
\textbf{Meena}: & \textit{I'd love to go to Japan, too.} \\
\textbf{Human}: & \textit{you're blocking me out! you have to talk to me} \\
\textbf{Meena}: & \textit{I'd love to go to Japan.} \\
\textbf{Human}: & \textit{where else?} \\
\textbf{Meena}: & \textit{I'd love to go to Japan, too!} \\
\bottomrule
\end{tabular}
\caption{Multiple near identical repetitions of \textit{``I'd love to go to Japan too."}.\label{t:rep1}}
\end{table}

\begin{table}
\small
\centering
\begin{tabular}{rp{6cm}}
\toprule
\multicolumn{2}{c}{{\bf Cross-turn Repetition Example 2}} \\
\midrule
\textbf{Human}: & \textit{Hi!} \\
\textbf{Meena}: & \textit{Hey there! How are you doing?} \\
\textbf{Human}: & \textit{not well, i'm quite depressed} \\
\textbf{Meena}: & \textit{That's no good. Wanna talk about it?} \\
\textbf{Human}: & \textit{not really, it'll only make it worse...can you cheer me up?} \\
\textbf{Meena}: & \textit{Sure! What's got you down?} \\
\textbf{Human}: & \textit{I'd love to hear a really lame joke} \\
\textbf{Meena}: & \textit{How about this one? What did the farmer say when he lost his tractor? Where is my tractor?} \\
\textbf{Human}: & \textit{haha that was lame! where did you hear it?} \\
\textbf{Meena}: & \textit{I was at the mall and I heard it in the food court. How was your day?} \\
\textbf{Human}: & \textit{wow, i didn't know you could walk!} \\
\textbf{Meena}: & \textit{Why did the scarecrow win an award?} \\
\textbf{Human}: & \textit{i don't know..you tell me!} \\
\textbf{Meena}: & \textit{Because he was outstanding in his field!} \\
\textbf{Human}: & \textit{haha, where did you hear that?} \\
\textbf{Meena}: & \textit{I was in the food court and I heard it in the field!} \\
\textbf{Human}: & \textit{you have a great sense of humor!} \\
\textbf{Meena}: & \textit{Why did the chicken cross the road? He was outstanding in his field!} \\
\textbf{Human}: & \textit{ok, i don't want to hear any more jokes} \\
\textbf{Meena}: & \textit{Do you know why he was outstanding in his field? Because he was a chicken!} \\
\textbf{Human}: & \textit{haha looks like you're really into this discussion!} \\
\textbf{Meena}: & \textit{Yes! I am! Do you know why? Because he was outstanding in his field!} \\
\textbf{Human}: & \textit{haha, borderline creepy but still funny :D} \\
\textbf{Meena}: & \textit{Why was the mouse trapped in the bag? Because he was outstanding in his field!} \\
\textbf{Human}: & \textit{i think i broke you} \\
\textbf{Meena}: & \textit{Do you know why I broke you? Because you were outstanding in your field!} \\
\bottomrule
\end{tabular}
\caption{Multiple partial repetitions of \textit{``(...) Because he was outstanding in his field!"}.\label{t:rep2}}
\end{table}

It is worth mentioning that there also exist in-turn contradictions and repetitions, where the contradiction or repetition is contained in the response turn itself (e.g., \textit{``I like pizza, but I don't like it"}). This type of artifact is often observed in Meena versions with worse perplexities, but is far less frequent in the \meenabase{}, which has the lowest perplexity as reflected in the samples shared in the appendix and the higher sensibleness scores.

We wrote a rule that detects if any two turns contain long common sub-sequences. We automatically remove candidates that are detected as repetition. This rule seems to have addressed most of the cross-turn repetition. We, therefore, further improve on the above interactive SSA of $74\% \pm \%1$ to $79\% \pm 1\%$.

\subsection{Safety Layer}
It is important to mention that the evaluation and conversation collection for the full Meena version was conducted with an additional classifier layer at serving time as part of the filtering mechanism to automatically filter out potentially sensitive or toxic response candidates for publication.

==> Towards a Human-like Open-Domain Chatbot/dataset.tex <==
The dataset used to train Meena is mined and filtered from public domain social media conversations.
The source data are essentially message trees involving multiple speakers: the very first message is the root; replies to a message are its child nodes. Any path along the tree induces a conversation where each message is a conversation turn. By treating each turn in a conversation path as a response and all the previous turns (up to 7) as a context, we create a training example of the form {\it (context, response)} pair.

We also filter the data to improve the generation quality.
A message is removed if any of the following conditions holds: 1.~the number of subwords is less than 2 or more than 128; 2.~the percentage of alphabetic characters is less than 70\%; 3.~message contains URL; 4.~author's username contains ``bot''; 
5.~the message is repeated more than 100 times;
6.~the message has a high $n$-gram overlap with the parent's text;
7.~the message is potentially unsafe or offensive with respect to a commercial text classifier.
In addition, we remove copies of the parent's text quoted in a message.

For simplicity, when a message is removed, we drop all sub-trees rooted under it. 
After these filtering steps, the number of $(context, response)$ pairs extracted is 867M. The text is tokenized using byte-pair-encoding (BPE)~\cite{senrich15} with the sentencepiece library.\footnote{\url{https://github.com/google/sentencepiece}} We use a vocabulary of 8K BPE subwords, which we found in our early experiments to be sufficient for generating specific responses while still allowing us to fit larger models in memory.

The final Meena dataset contains 341GB of text (40B words). In comparison, GPT-2 \cite{gpt2} has been trained on 40GB of Internet text (8 million web pages).


==> Towards a Human-like Open-Domain Chatbot/discussion.tex <==
Our results suggest perplexity on public domain social media conversations might be a good automatic proxy for human judgement of fundamental attributes of human-likeness, such as sensibleness and specificity. The results also suggests that optimizing the probability of the next token on larger volumes of social media conversations could lead to human-like sensibleness in an open-domain setting. However, our static evaluation dataset only contains one to three-turn contexts and is biased by the sources of the first turn and the fact that the two-turn and three-turn contexts build on the shorter contexts. Moreover the contexts in this dataset are predominantly Turing test and social conversation style, including common sense, basic knowledge, asking/sharing about personality, likes/dislikes, opinions, feelings, hobbies, pleasantries, etc. This dataset does not include contexts like deeper question answering (e.g., how fast is a cheetah), basic math (e.g., how much is 1+1) and common sense tests designed to challenge machines, but not humans \cite{levesque11}. Human-likeness is an incredibly broad and abstract concept. The interactive evaluation addresses some of the bias and scope limitations in static evaluation while still providing a consistent score to quantify a given chatbot. Nevertheless, unlike static evaluation it does not allow for granular comparison between different chatbot responses. In addition, it may be too short (14 to 28 turns), and may assign too much weight to typical beginning and ending of conversations. It may also be too short to cover deeper topics and exercise longer term memory.

Furthermore, it may be necessary to expand the set of basic human-like conversation attributes being measured beyond sensibleness and specificity. Some directions could include humor, empathy, deep reasoning, question answering and knowledge discussion skills. One could also break down sensibleness into its implicit sub-components: logical and personality consistency, common sense, relevance, basic factual correctness and so on. Future work may also explore the continued optimization of sensibleness via the optimization of test set perplexity.

==> Towards a Human-like Open-Domain Chatbot/evaluation.tex <==
Evaluating chatbots and natural language generation is a well-known challenge \citep{liu16, lowe17, novikova17, hashimoto19}, which we aim to address in this paper. First, we propose a human evaluation metric that captures key elements of human-likeness of conversational responses (Section 2.1). We then describe two human-evaluation setups: {\it static}, in which we benchmark models on a fixed set of multi-turn contexts to generate responses (Section 2.2); and {\it interactive}, where we allow humans to chat freely with chatbots (Section 2.4). Lastly, we detail our automatic evaluation metric for fast development and end-to-end optimization (Section 2.7).

\subsection{Measuring Human Likeness}
\label{subsec:metrics}

To measure the quality of a response given a context, we propose a sequence of two questions. We first ask whether the response, given the context, makes sense. Sensibleness arguably covers some of the most basic aspects of conversational human-likeness, such as common sense and logical coherence. Sensibleness also captures other important aspects of a chatbot, such as {\it consistency}. The crowd worker is asked to use common sense to judge if a response is completely reasonable in context. If anything seems off — confusing, illogical, out of context, or factually wrong — then it should be labeled as, ``does not make sense''.

However, being sensible is not enough. A generic response (e.g., \textit{I don't know}) can be sensible, but it is also boring and unspecific. Such responses are frequently generated by bots that are evaluated according to metrics like sensibleness alone \citep{li16diversity,amazoneval}. To illustrate this, we create GenericBot: a trivial bot that always replies to questions with ``I don't know" and to statements with ``ok" (examples in Appendix Table \ref{t:boring_bot_static_analysis}). On \textit{static} evaluation (using a fixed set of prompts and bot-generated responses), 70\% of GenericBot's responses are labeled sensible, surpassing even DialoGPT (62\%), even though DialoGPT is clearly more human-like than GenericBot. To overcome this issue, we need our evaluation to separate more fully human-like conversation from bland and generic statements. 
Therefore, if a response is labeled as sensible, we further ask the crowd worker to determine if it is specific to the given context. For example, if A says, ``I love tennis,'' and B responds, ``That's nice,'' then the utterance should be marked, ``not specific''. That reply could be used in dozens of different contexts. However, if B responds, ``Me too, I can't get enough of Roger Federer!'' then it is marked as ``specific'', since it relates closely to what is being discussed. Responses labeled not sensible are considered not specific. In GenericBot's case, none of the responses are specific, whereas 39\% of DialoGPT's responses are specific.

This sequence of two questions is designed to start with the most concrete and basic human quality (sensibleness) and then progress to the arguably more subjective human quality (specificity). The degree of subjectivity is somewhat quantified in the crowd worker agreement. We measure crowd worker consistency for every model benchmark using agreement and Krippendorff's alpha~\cite{krippendorff15}, shown in Table \ref{t:rater_consistency}. The agreement is reasonable considering the questions are subjective and the final results are always aggregated labels (e.g., average sensibleness across all chatbot responses).

\begin{table}[h!]
\small
\centering
\begin{tabular}{c|c|c}
\toprule
{Metric} & {\bf Agreement (\%)} & {\bf Krippendorff's alpha} \\
\midrule
Sensibleness & $76 \pm 3$ & $0.42 \pm 0.03$ \\
\midrule
Specificity & $66 \pm 2$ & $0.30 \pm 0.05$  \\
\bottomrule
\end{tabular}
\caption{The average and standard deviation of crowd worker agreement across static evaluations of Meena models. Each static evaluation consisted of 1,477 $(context, response)$ pairs, each labeled by 5 crowd workers.}
\label{t:rater_consistency}
\end{table}

Given a set of responses labeled as described above, we can calculate sensibleness and specificity as the percentage of responses labeled as sensible and specific, respectively. To combine these two into one metric, we take a simple average of the two, which we call SSA (\textbf{s}ensibleness and \textbf{s}pecificity \textbf{a}verage). SSA is a proxy for human likeness, which also penalizes chatbots that consistently produce generic responses. For example, GenericBot's SSA is 35\% and DialoGPT's SSA is 51\%, providing a much more fair separation and ranking than sensibleness alone.

Before arriving at SSA, and before any of the chatbots were tested, the authors of this paper conducted several rounds of pilot studies on what to ask crowd workers and how to best phrase the instructions. We settled on the two-question SSA for several reasons: it was easy for crowd workers to understand; alternative additional questions did not add extra information; and more subjective questions result in lower agreement between crowd workers.

As an additional check on the SSA metric, we reran a static evaluation, this time asking crowd workers to assess whether or not a response is ``humanlike''. We find that there is a high correlation between those labels and the two components of the SSA metric (Figures \ref{fig:ssa-human-likeness}, \ref{fig:sensibleness-human-likeness}, \ref{fig:specificity-human-likeness}). Compared to a direct evaluation of what crowd workers consider to be ``humanlike'', SSA has significant advantages for large-scale evaluation tasks: it is more objective, easier for crowd workers to understand, and penalizes boring and vague responses. Nevertheless, these findings give us confidence that SSA is indeed capturing important aspects of human likeness.

\begin{figure}
\centering
\includegraphics[height=150pt]{fig/ssa-human-likenesss.pdf}
\caption{SSA vs human likeness. Each point is a different chatbot, except for the top right one, which is human. A regression line is plotted, for which the coefficient of determination ($R^2$) is 0.96. The SSA values were collected using static evaluation mode (Section \ref{subsec:ssa}). The human likeness evaluation was also conducted in static evaluation mode. Instead of judging sensibleness or specificity, however, we asked crowd workers to judge whether a given response was ``human-like", or in other words, looked like a response that a human might give in the provided context.
}
\label{fig:ssa-human-likeness}
\end{figure}

\subsection{Static Evaluation}
\label{subsec:ssa}
In order to have a common benchmark to easily compare models, we create a collection of
1,477 conversational contexts with between 1 and 3 conversation turns, that we call the Mini-Turing Benchmark (MTB).
We started this dataset by compiling single-turn contexts (e.g., ``How are you?") from multiple sources, such as from the work\footnote{\url{http://ai.stanford.edu/~quocle/QAresults.pdf}} of~\citet{vinyals15} and the transcripts of the Loebner Prize\footnote{\url{https://aisb.org.uk/events/loebner-prize}} contests (years 2014-2018).
In total, there were 315 single-turn contexts, which we then extended to include 500 two-turn and 662 three-turn contexts.
 
The MTB also contains contexts with personality questions (e.g. ``Do you like cats?''), some of which expect responses with personality consistency. For example, the context ``A: Do you like movies?; B: Yeah. I like sci-fi mostly; A: Really? Which is your favorite?'' expects a consistent response such as \textit{I love Back to the Future}. On the other hand, a response like \textit{I don't like movies} would be a contradiction, and thus not considered sensible.

When evaluating chatbots, all MTB contexts are fed to the models or presented to humans to obtain responses. We send the resulting $(context, response)$ pairs to crowd workers and asked whether each response given the context is sensible and specific as defined in \ref{subsec:metrics}. We call this {\it static evaluation} because the contexts are fixed.

\subsection{Interactive Evaluation}
\label{subsec:interactive}
Static evaluation may be suitable for comparing models, but it is biased by how the static evaluation dataset was constructed. To address this, we create an additional evaluation mode where the crowd workers can chat 1:1 with a chatbot about anything they want. As with static evaluation, workers are also asked to decide whether each response from the chatbot is sensible and specific as defined in \ref{subsec:metrics}. Conversations start with ``Hi!'' from the chatbot to mark the beginning of the conversation and crowd workers have no expectation or instructions about domain or topic of the conversation. A conversation is required to last at least 14 turns (7 from chatbot) and at most 28 turns. We collected 100 such conversations for each model (i.e., at least 700 labeled turns per model). We then measure the percentage of labeled turns that are sensible and specific.

Unlike a typical Turing test~\citep{turing50}, we tell the human judges upfront that they are about to chat with an experimental chatbot and ask them to label what the chatbot says in terms of sensibleness and specificity. This shifts the focus of the judges and chatbot creators from optimizing for deception detection to optimizing for detecting and maximizing human-like qualities (e.g., sensibleness). Similar to our approach, \citet{asma19} also conduct interactive evaluation by allowing humans to chat freely with bots. Their setup, however, focuses on evaluating conversations as a whole (as opposed to at the level of individual turns) and judges evaluate for quality, fluency, diversity, relatedness, and empathy.

\subsection{Estimate of Human Performance}
To estimate static SSA of humans we ask crowd workers to respond to MTB contexts. Additionally, to estimate human interactive SSA, we leveraged the help of internal company volunteers to collect 100 human-human conversations following mostly the same instructions as crowd workers for every other chatbot. Labeling of sensibleness and specificity was conducted by independent crowd workers with majority voting of 5 workers per human turn. The difference from the rest of the evaluations is that, in this case, participants knew they were chatting with another human. In contrast, when humans chat with a chatbot they will occasionally say unusual things to test the chatbot's limits. \citet{hill15} describe differences in human behavior when talking to a chatbot. That said, we never incentivize humans to chat adversarially with chatbots in any of our evaluations.

\subsection{Evaluation of Cleverbot and DialoGPT}
\label{sec:cleverbot_dialogpt_eval}
To integrate with Cleverbot, we leverage its API. For DialoGPT, we use its open sourced 762M parameter model.\footnote{\url{https://github.com/microsoft/DialoGPT}} It is worth mentioning that we initially tried the 345M parameter DialoGPT model, because it was reported to perform best on single-turn human evaluation. However, the 345M parameter model seemed to perform noticeably worse than the 762M one in preliminary evaluations of multi-turn conversations. Our human evaluation is multi-turn, so we select the 762M model.

The DialoGPT authors were unable to release their decoding script at the time of writing. Therefore, following their published description, we use top-K decoding with $K=10$. We adapt the decoding implementation by \citet{wolf19}. Moreover, since the backward model was also not released we were not able to try their MMI re-ranking~\citep{li16diversity}.

Both Cleverbot and DialoGPT were evaluated using the same crowd sourcing setup as for Meena.

\subsection{Evaluation of Mitsuku and XiaoIce}
\label{sec:xiaoice_mitsuku_eval}
Because we chose to use the free Mitsuku web app\footnote{Pandorabots offers a paid enterprise package, which includes the Mitsuku API.}, and there is no public API for XiaoIce, we called on the help of internal company volunteers and only conducted interactive evaluation. Volunteers collectively had 100 conversations with Mitsuku, and 119 with XiaoIce on their publicly available web apps. The volunteers conversed with the chatbots following mostly the same instructions that crowd workers follow for every other chatbot. The difference is that humans would say ``Hi!" for the first turn, instead of the chatbot, in order to keep the first turn the same as other cases. Labeling of sensibleness and specificity in all cases was conducted by independent crowd workers with majority voting of 5 workers per chatbot turn. Also note that both XiaoIce and Mitsuku sometimes include an image in their reply and occasionally, volunteers include text descriptions of the images they see. The presence of the image may in some cases change the sensibleness of the response for better or worse.

XiaoIce interacts in Mandarin so both the volunteers and the independent crowd workers were native Mandarin speakers. The group of volunteers for XiaoIce, Mitsuku, and human-human conversations were mostly disjoint. Other than requiring a knowledge of Mandarin for XiaoIce conversations, volunteer selection was arbitrary. We had 29 volunteers for XiaoIce, 43 for Mitsuku, and 21 for human-human.

To reset Mitsuku state between conversations, volunteers refreshed the web page. During the writing of this paper there was no clear way to reset the state of XiaoIce. The XiaoIce team have informed us that not resetting the state negatively affects the model's control of the context.\footnote{From personal communication with the XiaoIce team, after the writing of the paper.} Also, most XiaoIce volunteers shared the same Weibo account.\footnote{Weibo is a microblogging service mostly used in China, which also allows users to chat with XiaoIce: \url{https://www.weibo.com/}} The XiaoIce team confirmed that account reuse negatively impacts the internal profile constructed by XiaoIce for a user. The XiaoIce team further suggested that, if the same Weibo account needs to be reused, we should wait at least one hour between volunteers using the account. In our experiments, we may have sometimes waited less than that amount of time between volunteers, although we made sure the account was only used by one volunteer at a time. Finally, the XiaoIce team mentioned that in the past few months (as of this writing), a limited version of XiaoIce with the smallest index has been served on Weibo. This version is expected to produce less satisfactory responses.

Direct comparisons between XiaoIce and other chatbots come with a caveat: XiaoIce can be seen as a product that optimizes for long-term user engagement, of which dialog generation is just one component. In other words, Meena is arguably at an advantage when comparing SSA scores.

\subsection{Automatic Evaluation}
\label{subsec:auto}
For quick research iterations, we focus on perplexity. Unlike the previous two evaluation types, perplexity is an automatic metric. A seq2seq model outputs a probability distribution over possible next response tokens. Perplexity measures how well the model predicts the test set data; in other words, how accurately it anticipates what people will say next. When interpreting perplexity scores, bear in mind that lower is better and that the theoretical minimum is one.

As shown in Section \ref{sec:results}, this commonly used metric correlates with human judgement of sensibleness and specificity. This is encouraging, because it is both automatic and directly optimizable with the standard cross-entropy loss function.

==> Towards a Human-like Open-Domain Chatbot/intro.tex <==
\begin{figure}[ht]
\centering
\includegraphics[height=150pt]{fig/ppl-issa.pdf}
\caption{Interactive SSA vs Perplexity. Each point is a different version of the Meena model. A regression line is plotted, for which the coefficient of determination ($R^2$) is 0.93, an indication of strong correlation between perplexity and the human evaluation metric (SSA). The dotted lines show the SSA performance of other chatbots, humans (86\%), the best end-to-end trained Meena model (72\%), and the full version of Meena which incorporates a filtering mechanism and tuned decoding (Section \ref{sec:advance_ssa}) and scores 79\%. Mitsuku and Cleverbot scored the same on overall SSA, but Mitsuku displayed higher sensibleness, whereas Cleverbot had higher specificity. See Sections \ref{sec:cleverbot_dialogpt_eval}, \ref{sec:xiaoice_mitsuku_eval}, and \ref{sec:results_other_bots} for more details on how we performed these comparisons and how to interpret the results.\label{fig:ppl-issa}}
\end{figure}

The ability to converse freely in natural language is one of the hallmarks of human intelligence, and is likely a requirement for true artificial intelligence. In order to explore this aspect of intelligence, many researchers are working on open-domain chatbots. Unlike closed-domain chatbots, which respond to keywords or intents to accomplish specific tasks, open-domain chatbots can engage in conversation on any topic. Some open-domain chatbots such as MILABOT~\cite{milabot}, XiaoIce~\cite{xiaoice}\footnote{\url{https://www.msxiaobing.com/}}, Gunrock~\cite{gunrock}, Mitsuku~\cite{mitsuku18}\footnote{\url{https://www.pandorabots.com/mitsuku/}} and Cleverbot\footnote{\url{https://www.cleverbot.com/}} (by Rollo Carpenter) display human-like attributes, but rely on complex frameworks, such as dialog managers with knowledge-based, retrieval-based, or rule-based systems. End-to-end neural network approaches \cite{shang15,vinyals15,sordoni15,serban16,dialogpt}, on the other hand, offer the simplicity of a single learned model.\blfootnote{Conversations with Meena, and with various other chatbots, are available at \url{https://github.com/google-research/google-research/tree/master/meena/}} Despite much research, open-domain chatbots still have weaknesses that prevent them from being generally useful: they often respond to open-ended input in ways that do not make sense, or with replies that are vague and generic.

Here we present Meena, a generative chatbot model that was trained end-to-end on 40B words mined and filtered from public domain social media conversations. With Meena, we push the limits of the end-to-end approach and show that a large-scale low-perplexity model can be a good conversationalist. We use a seq2seq model~\citep{sutskever14,bog15} with the Evolved Transformer~\citep{et} as the main architecture. The model is trained on multi-turn conversations where the input sequence is all turns of the context (up to 7) and the output sequence is the response. Our best model has 2.6B parameters and achieves a test perplexity of \bestppl{} based on a vocabulary of 8K BPE subwords~\cite{senrich15}.

To measure the quality of Meena and other chatbots, we propose a simple human evaluation metric. Sensibleness and Specificity Average (SSA) combines two fundamental aspects of a human-like chatbot: making sense and being specific. We ask human judges to label every model response on these two criteria. The first part of the metric, sensibleness, is a basic requirement. To converse properly with a human, a bot's responses have to make sense in context; humans typically take this for granted when conversing with one another, and our evaluations find that 97\% of  human-produced statements meet this criterion (see Section~\ref{sec:human_level}). However, making sense is not enough. If a model is designed with sensibleness as its only objective, its responses could be vague and boring, since that is a safe strategy to avoid being penalised for not making sense. For example, closed-domain chatbots typically respond with a generic apology when a human asks something outside their domain; some end-to-end learned chatbots respond ``I don't know'' to many inputs \citep{li16diversity}; and Turing Test contest entrants often try to avoid detection by being strategically vague \citep{amazoneval}. They succeed in not generating gibberish or contradicting themselves, but at the cost of not really saying anything of substance. To mitigate this, we add a second dimension to the SSA metric, which asks our evaluators whether a response is specific given the context. This prevents bots from hiding behind vague replies, allowing us to more openly examine what they are capable of. As discussed in Section~\ref{subsec:metrics}, this successfully distinguishes between generic and lively responses, while also being simple and easy for crowd workers to understand.

We compare Meena, humans, and other open-domain chatbots using the SSA metric with two types of human evaluation: \textit{static} and \textit{interactive}. For static evaluation, we curated a dataset with 1,477 multi-turn conversations. For interactive evaluation, humans could chat about anything they wanted. We were surprised, but pleased, to discover that the SSA metric shows strong correlation with Meena's perplexity, both in static and interactive evaluation. In other words, the better that Meena fit its training data, the more sensible and specific its chat responses became. At first glance, this result may seem intuitive, but it surprised us because recent research found a poor correlation between human evaluation scores and automatic metrics such as BLEU \citep{liu16,lowe17}.

Our best end-to-end learned model has an average of 72\% SSA. The full version of Meena scores 79\% by incorporating a filtering mechanism and tuned decoding (Section \ref{sec:advance_ssa}). This is still below the \humanissa\% SSA achieved by an average human, but is far closer than the other chatbots we tested. We note that humans have very high sensibleness, but significantly lower specificity, as detailed in Section \ref{sec:human_level}.

We will also discuss weaknesses of our methodology. For example, our static evaluation dataset is too restricted to capture all aspects of human conversations. Nevertheless, the fact that Meena achieves such a high SSA score and that there is a correlation between SSA and perplexity means that a human-like chatbot, in terms of sensibleness and specificity, could be in sight if we can attain better perplexity.

Our contributions are: (1) proposing a simple human evaluation metric for multi-turn open-domain chatbots that captures basic, but important, attributes of human conversation; (2) showing evidence that perplexity is an automatic metric that correlates with human judgment, in contrast to recent findings on other automatic metrics mentioned above; (3) demonstrating that an end-to-end neural model with sufficiently low perplexity can surpass the sensibleness and specificity of existing chatbots that rely on complex, handcrafted frameworks developed over many years.

==> Towards a Human-like Open-Domain Chatbot/meena.tex <==
\begin{table*}[tbh!]
\small
\centering
\begin{tabular}{p{12cm}|>{\centering\arraybackslash}p{1cm}}
\toprule
\multicolumn{1}{c|}{{\bf Responses} for \turn{Why do you like the ocean?}} & {\bf Score} \\
\midrule
1. I love the beach. I like that it doesn't have anything in it. Just open water. & -12.98 \\
2. It's dark and mysterious. I discovered it when I was really young and it was a dream of mine since. The ocean is full of wonders, mysteries and great things to discover. I love snorkeling. I moved to Hawaii a year ago and I'm going to college for marine biology. So there's that. & -14.03 \\
3. The sea sounds cool and it's really satisfying to swim in. & -14.62 \\
4. I dunno. It's beautiful, I guess. It reflects my upbringing, I reckon. & -14.87 \\
5. Well I'm from the pacific northwest and always somehow end up back there. I've been to Hawaii but I'm not one for the beach, it's too hot and the air is so dry. & -15.36 \\
6. The beauty of it is incredible, and swimming in it and being able to see huge waves sweeping by is just amazing. I was born in the desert so it's really the only place in the world I've seen with flowing water around me & -17.07 \\
7. It's beautiful, maybe? I just wish I lived closer to it! & -17.14 \\
8. It's pretty and soothing. & -17.19 \\
9. Because I love the smell. I love walking when I can through the beach. I live in California so I basically go to the ocean almost every weekend. & -17.38 \\
10. The ocean is pretty cool, I suppose. I like the various types of fish. & -17.90 \\
\bottomrule
\end{tabular}
\caption{{\bf Sampling Outputs} -- responses found by sampling with temperature, sorted by the length-normalized log-likelihood scores and using the same Evolved Transformer as the one used in Table~\ref{t:beam}. The scores are calculated as $\frac{\log P}{T}$, where $P$ is the likelihood of the response and $T$ is the number of tokens.}
\label{t:sampling}
\end{table*}

\begin{table}
\small
\centering
\begin{tabular}{p{6cm}|c}
\toprule
\multicolumn{1}{c|}{{\bf Responses} for \turn{Why do you like the ocean?}} & {\bf Score} \\
\midrule
1. Why don't you like the ocean? & -1.70 \\
2. I don't like the ocean. I love the ocean. & -2.66 \\
3. I don't like the ocean. I love it. & -2.78 \\
4. I don't like the ocean, I love the ocean. & -2.94 \\
5. I don't like the ocean, I love it. & -2.94 \\
6. Why don't you like the ocean? :P & -2.95 \\
7. I don't like the ocean, I love it! & -3.15 \\
8. I don't like the ocean. I love the ocean! & -3.20 \\
9. Why don't you like the ocean? It's beautiful. & -3.26 \\
10. I don't like the ocean. I love the ocean. There's a difference. & -3.31 \\
\bottomrule
\end{tabular}
\caption{{\bf Beam Search Outputs} -- top responses generated by beam-search decoding and the corresponding length-normalized log-likelihood scores. We use an Evolved Transformer with perplexity 10.2 and vocabulary size of 8K.}
\label{t:beam}
\end{table}

As described above, recent work on end-to-end dialog models has fallen into two broad categories: (1) complex models with human-designed components, and (2) large neural network models (known as end-to-end models) that are closer to generic learning frameworks. End-to-end models have shown promise, but clear limitations \cite{gao19}. An open question has been: in order to reach a point where a model can carry out high-quality, multi-turn conversations with humans, could we simply take an end-to-end model and make it bigger---by adding more training data and increasing its parameter count---or is it necessary to combine such a model with other components? In this section we describe the Meena model, the largest end-to-end model to enter the field so far. We believe it answers the open research question, by showing that a large end-to-end model can generate almost humanlike chat responses in an open-domain setting.

In this section, we will describe the training data, architecture, and decoding algorithm. We will also provide a few sample conversations that Meena has had with humans. 

\subsection{Training Data}
\label{sec:dataset}
\input{dataset.tex}

\subsection{Model Architecture}
The best performing Meena model is an Evolved Transformer (ET)~\citep{et} seq2seq model with 2.6B parameters, which includes 1 ET encoder block and 13 ET decoder blocks. The Evolved Transformer is an evolutionary NAS architecture~\citep{real17,real18} based on the Transformer~\cite{transformer}. Our largest (i.e., maximum memory usage) Evolved Transformer scored 10.2 perplexity and our largest vanilla Transformer scored perplexity 10.7 for the same number of training steps (738k). The largest vanilla Transformer had 32 decoder layers with other architectural hyperparameters held constant.\footnote{An Evolved Transformer block is about twice as deep as a Transformer layer}

For comparison, the extra-large GPT-2 model~\cite{gpt2} has 1.5B parameters and is a language model (i.e., decoder only); whereas the large conversational model from the recent DialoGPT work~\cite{dialogpt} has 762M parameters.

Meena's hidden size is 2,560 and the number of attention heads is 32. We share the embeddings across the encoder, the decoder, and the softmax layer. The encoder and decoder each have a maximum length of 128 tokens (i.e., 256 combined). The hyperparameters of our best model were found via manual coordinate-descent search.

\subsection{Training Details}
We trained our best model for 30 days on a TPU-v3 Pod (2,048 TPU cores) on the Meena dataset containing 40B words (or 61B BPE tokens). Interestingly, the 2.6B-parameter model can overfit~\footnote{In the sense that validation loss increases as train loss decreases.} on a 61B-token dataset which suggests a surprisingly large model capacity.
Therefore, we add a small amount of 0.1 attention and feed-forward layer dropout. Additionally, to save memory, we chose the Adafactor optimizer~\cite{shazeer18} with 0.01 as the initial learning rate, keeping it constant for the first 10k steps and then decaying with the inverse square root of the number of steps. We use the Tensor2Tensor codebase~\cite{tensor2tensor} for training Meena.\footnote{\url{https://github.com/tensorflow/tensor2tensor}}

A TPU-v3 core has 16GB of high-bandwidth memory. We maximized memory usage for model parameters and stored only 8 training examples per core. Each training step took about 1 second. In the full TPU-v3 Pod, this meant we learned over 4M tokens per training second. Therefore, by the end of training, the model had traversed the full training set 164 times (or epochs) and observed a total of about 10T tokens (including repeated ones).

\subsection{Decoding}
\label{meena-decoding}

Generating generic (i.e., not specific) and bland responses \citep{li16diversity} has always been a major challenge in existing neural conversational models. A common approach to mitigating this problem is to use more sophisticated decoding algorithms, for instance with different forms of re-ranking \citep{li16diversity,shao17} or conditioning on profiles, topics, and styles \citep{li16,wang17,xing17,zhang18personal}. Recent works also explore new frameworks such as adversarial learning \citep{li17adversarial,zhang18}, variational autoencoding \citep{zhao17,gu19}, or both \citep{gao19joint} at the cost of added complexity and less scalability.

In contrast, we show that given a model with sufficiently low perplexity, a simple sample-and-rank decoding strategy achieves both diverse and high-quality responses. Sample-and-rank, works as follows: First, we sample $N$ independent candidate responses using plain random sampling with temperature $T$. Second, we select the candidate response with the highest probability to use as the final output.

Temperature $T > 0$ is a hyper-parameter that regulates the probability distribution $p_i$ of the next token during decoding. We divide the logits $z_i$ by $T$ before computing the ``softmax" as in \citet{hinton15}:

\begin{equation}
p_i = \frac{\exp(z_i/T)}{\sum_{j}\exp(z_j/T)}
\end{equation}

$T=1$ yields the unmodified distribution. We observe that large values of $T$ favor contextually rare tokens, such as relevant entity names, but might also assign too much probability to incorrect tokens depending on the model's predictions. Meanwhile, smaller values of $T$ favor more common words such as articles or prepositions, which are safer but less specific.

Tables~\ref{t:sampling} and \ref{t:beam} show responses for the arbitrary probing input \turn{Why do you like the ocean?} under sample-and-rank and beam-search, respectively.
As we can see, beam-search decoding generates repetitive and uninteresting responses. On the other hand, sample-and-rank provides us with diverse and content-rich responses. The key here is to have a model with low perplexity so samples can be taken at high temperature to produce human-like content.

For all the results in Section~\ref{sec:results}, we use sample-and-rank with $N=20$ and $T=0.88$. Additionally, as shown in Figure~\ref{fig:ppl-issa}, for this fixed decoding strategy, sensibleness and specificity improve as model test set perplexity falls. For additional decoding results and samples, see Section~\ref{sec:advance_ssa}.

\FloatBarrier
\subsection{Sample conversations}
\label{sec:sample_conversations}
Below are cherry picked conversations that Meena has had with humans. We selected these conversations \textit{after} they were completed. That is, the Meena responses within the conversations were not cherry picked; they were produced automatically using sample-and-rank (Section \ref{meena-decoding}). Conversations B and C are excerpts from conversations number 43 and 48, respectively, of the conversations dataset published on GitHub.\footnote{\url{https://github.com/google-research/google-research/tree/master/meena/}}

\vspace{3em}
\begin{table}[ht!]
\small
\centering
\begin{tabular}{rp{6cm}}
\toprule
\multicolumn{2}{c}{{\bf Conversation A}} \\
\midrule
\textbf{Human}: & \textit{say you're in an empty giant office and you see a black bird flying indoors. what do you do?} \\
\textbf{Meena}: & \textit{What kind of bird? Is it friendly? How large? How big is the office? Is it indoors or outdoors?} \\
\textbf{Human}: & \textit{well it's a predator bird and it's gonna eat you} \\
\textbf{Meena}: & \textit{I would grab my phone and call 911.} \\
\bottomrule
\end{tabular}
\caption*{Meena handles arbitrary open-domain input. However, asking ``Is it indoors or outdoors" was not sensible. \label{t:conv4}}
\end{table}

\begin{table}[ht]
\small
\centering
\begin{tabular}{rp{6cm}}
\toprule
\multicolumn{2}{c}{{\bf Conversation B}} \\
\midrule
\textbf{Human}: & \textit{Hi!} \\
\textbf{Meena}: & \textit{Hi! How are you this fine evening?} \\
\textbf{Human}: & \textit{I'm doing well. it's morning my time!} \\
\textbf{Meena}: & \textit{Good morning! What are your plans for today?} \\
\textbf{Human}: & \textit{Get my work done then watch a movie at home in the night} \\
\textbf{Meena}: & \textit{Sounds fun! What movie?} \\
\textbf{Human}: & \textit{I haven't decided yet, perhaps an Oscar-nominated one. any suggestion?} \\
\textbf{Meena}: & \textit{I'm not too familiar with recent Oscar winners, but I do know I wanted to see The Grand Budapest Hotel.} \\
\textbf{Human}: & \textit{ah, tell me about that movie!} \\
\textbf{Meena}: & \textit{It's from the same director and writer as Moonrise Kingdom. Wes Anderson is pretty well known for making funny, colorful films. I've heard it's pretty good.} \\
\textbf{Human}: & \textit{ha! I've searched on the internet and both movies are very colorful!} \\
\textbf{Meena}: & \textit{I'm looking forward to it. I love colorful movies.} \\
\bottomrule
\end{tabular}
\caption*{The Grand Budapest Hotel and Moonrise Kingdom are indeed colorful movies, directed by Wes Anderson.\label{t:conv1}}
\end{table}

\begin{table}[ht!]
\small
\centering
\begin{tabular}{rp{6cm}}
\toprule
\multicolumn{2}{c}{{\bf Conversation C}} \\
\midrule
\textbf{Human}: & \textit{Haha, I think mathematics has a presence beyond human existence.} \\
\textbf{Meena}: & \textit{So does philosophy.} \\
\textbf{Human}: & \textit{Can you state with examples how this is true.} \\
\textbf{Meena}: & \textit{Can you state how it isn't?} \\
\textbf{Human}: & \textit{Without human existence there will be no one left to comprehend whats right whats wrong, and thus philosophy wi [sic]} \\
\textbf{Meena}: & \textit{That's not the definition of philosophy.} \\
\textbf{Human}: & \textit{Without human existence there will be no one left to comprehend whats right whats wrong, and thus philosophy will not be needed. How do you define philosophy?} \\
\textbf{Meena}: & \textit{The study of general knowledge or the fundamental nature of things.} \\
\bottomrule
\end{tabular}
\caption*{Meena tries to define philosophy.\label{t:conv3}}
\end{table}

\begin{table}[ht!]
\small
\centering
\begin{tabular}{rp{6cm}}
\toprule
\multicolumn{2}{c}{{\bf Conversation D}} \\
\midrule
\textbf{Human}: & \textit{I like how cute cows are} \\
\textbf{Meena}: & \textit{Ah, interesting. You like how they are cute, right?} \\
\textbf{Human}: & \textit{yeah, and they're realy smart} \\
\textbf{Meena}: & \textit{I heard they go to college} \\
\textbf{Human}: & \textit{cows go to college?} \\
\textbf{Meena}: & \textit{I heard that a cow went to Harvard.} \\
\textbf{Human}: & \textit{what did the cow study?} \\
\textbf{Meena}: & \textit{Bovine sciences.} \\
\textbf{Human}: & \textit{do horses go to Harvard?} \\
\textbf{Meena}: & \textit{Horses go to Hayvard.} \\
\textbf{Human}: & \textit{that's a pretty good joke, I feel like you led me into it} \\
\textbf{Meena}: & \textit{You were trying to steer it elsewhere, I can see it.} \\
\bottomrule
\end{tabular}
\caption*{Meena executes a multi-turn joke in an open-domain setting. We were unable to find this in the data.\label{t:conv2}}
\end{table}

\FloatBarrier

Appendix \ref{apdx:conversations} shows random samples of conversations.

==> Towards a Human-like Open-Domain Chatbot/related.tex <==
Finding a good automatic metric that correlates with human evaluation has been an important goal of open-domain conversational modeling. BLEU~\cite{Papineni02bleu}, ROUGE~\cite{rouge}, or other related metrics in translation and summarization, while popular and easy to compute, have been shown to be unsuitable for dialog \citep{liu16} or more broadly language generation systems \cite{novikova17}.

Past works have attempted to build learnable metrics, either in a supervised fashion~\cite{lowe17}, which requires human labels, or with unsupervised approaches~\cite{ruber,ghazarian19}, that are more complex and need separate training, e.g., of a ranking system. In our work, we show that perplexity, which is readily available to any neural seq2seq model, exhibits a strong correlation with human evaluation.
Our work is therefore also related to past attempts to correlate perplexity with other automatic metrics
in other tasks, e.g., perplexity vs.~BLEU in translation~\cite{luong15}.

Another interesting line of work is to combine human evaluation with either automatic metrics~\cite{chaganty18} or with model likelihood~\cite{hashimoto19}. While theoretically motivated, these metrics are too complex to be practical, requiring both human judgments and training separate models, e.g., an estimator~\cite{chaganty18} to reduce bias in automatic evaluation or a discriminator~\cite{hashimoto19} to distinguish between human- and model-generated samples.

In terms of designing of human evaluation metrics, existing literature differs in what attributes are used to assess the quality of a neural conversational model. Many works, e.g., \citet{zhao17,xu18,ippolito19}, have focused solely on the diversity aspect to counter the commonly observed problem of models generating generic responses \cite{li16diversity}.
Others have attempted to improve and evaluate multiple aspects at once. For example, 
\citet{amazoneval} aim to unify many metrics, such as diversity, engagement, and user experience; \citet{gao19joint} jointly optimize for both diversity and relevance; \citet{see19} control decoding attributes (such as repetition, specificity, response-relatedness, and question-asking) to improve engagingness and interestingness; and \citet{hashimoto19} design metrics to capture human likeness and diversity.

In contrast, we focus on sensibleness and specificity for our human evaluation. 
While human likeness and relevance used in aforementioned works are related to sensibleness, we specifically use sensibleness as it leads to better agreement among crowd workers (see $\S$\ref{subsec:metrics}). 
Similar reasoning applies to specificity, which is related to other attributes such as engagingness and interestingness, as measured in previous works.\footnote{It is worth pointing out that we do not explicitly measure diversity as it requires judging a set of responses; whereas, for conversation, what is most important is the first reply that a chatbot produces.
As our decoding method is sampling, it implies that our generation is diverse. However, there remains a question of whether the sampled response is of high quality. The fact that our model has low perplexity and achieves high SSA score indicates that the generation is meaningful.
}
A limitation of our work is that it does not cover aspects such as empathy \cite{xiaoice,rashkin18}.

While we do not explicitly control for specificity, existing works, such as \cite{zhang18control,ko19}, attempted to do so by augmenting the decoder of seq2seq models with specificity-control components. These added complexities sometimes lead to implausible responses as analyzed by \citet{ko19}. In contrast, the specificity of our model improves as perplexity decreases.

Recent work on DialoGPT \cite{dialogpt} compares the conversation quality of chatbots with that of humans but their evaluation settings are limited to single-turn dialogs. We instead conduct our evaluation on conversations of up to 3 turns in the static MTB benchmark and 14 turns in the interactive setup.

==> Towards a Human-like Open-Domain Chatbot/results.tex <==
In this section, we will first demonstrate the correlation between test perplexity and the human evaluation metric, SSA, defined earlier. We also include human-level upperbound estimates for both static and interactive evaluations, beside performances of other chatbots, such as XiaoIce, Mitsuku, DialoGPT, and Cleverbot. Lastly, we provide sample responses for different models given the same contexts to understand how Meena qualitatively compares to others.

\begin{figure}[tbh!]
\centering
\begin{minipage}{0.45\textwidth}
  \centering
  \includegraphics[height=150pt]{fig/ppl-isensibleness.pdf}
  \caption{Interactive sensibleness vs perplexity.\label{fig:ppl-isensibleness}}
\end{minipage} \hfill
\begin{minipage}{0.45\textwidth}
  \centering
  \includegraphics[height=150pt]{fig/ppl-ispecificity.pdf}
  \caption{Interactive specificity vs perplexity.\label{fig:ppl-ispecificity}}
\end{minipage}
\end{figure}

\subsection{SSA-perplexity correlation}
We trained models with different hyper-parameter settings and architectures on the dataset described in Section \ref{sec:dataset}. We vary the number of layers, attention heads, total training steps, whether we use Evolved Transformer or regular Transformer and whether we train with hard labels or soft labels/distillation \cite{hinton15}. The trained models are then measured with an automatic metric, test perplexity (Section \ref{subsec:auto}), and also with human metrics (\Cref{subsec:ssa,subsec:interactive}). Our results indicate most of the variance in the human metrics can be explained by the test perplexity. The end-to-end trained Meena model with lowest perplexity is referred to as {\it \meenabase{}}. In addition, we also include an improved version of Meena (detailed in Section 5) and refer to this as the {\it{\meenafull{}}} model, or just {\it{Meena}} model for short.

\begin{figure*}[tbh!]
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=1.0\textwidth]{fig/ppl-ssa.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=1.0\textwidth]{fig/ppl-sensibleness.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=1.0\textwidth]{fig/ppl-specificity.pdf}
    \end{subfigure}
    \caption{Static evaluation results.\label{fig:static-evaluation}}    
\end{figure*}

The correlation was $R^2=0.93$ for static sensibleness vs perplexity and $R^2=0.94$ for static specificity vs perplexity indicating this might be a good automatic metric for measuring sensibleness and specificity. Static SSA vs perplexity has $R^2=0.94$. The static evaluation results are shown in Figure \ref{fig:static-evaluation}. The correlation is close to linear, but it is unclear whether the trend will continue for even lower values of perplexity.

In interactive evaluation (Section \ref{subsec:interactive}) crowd workers could chat about anything they wanted. We observe similarly strong correlation with perplexity (see \Cref{fig:ppl-isensibleness,fig:ppl-ispecificity,fig:ppl-issa}) and very similar sensibleness and specificity values as the static evaluation. This indicates that the static evaluation correlation with perplexity is not due to dataset bias.

Regarding consistency, the lowest perplexity model was evaluated 7 times with static evaluations and also 7 times with interactive evaluations. Each time, we obtained a different set of randomly sampled responses. Across the evaluations the standard deviation is $2\%$ for static SSA and is $1\%$ for interactive SSA, indicating that both metrics are consistent enough for our purposes.

\subsection{Human-level Estimates}
\label{sec:human_level}
As expected, human sensibleness is very high, but it is not perfect. Human sensibleness was estimated at 94\% static and 97\% interactive. People have misunderstandings, miss attempts at humor and sometimes lack shared context or background. Also aligned with intuition, humans are sometimes not specific due to momentary lack of ideas, interest or knowledge. The human specificity scores are 69\% static and 75\% interactive. The resulting SSAs are 82\% static and 86\% interactive.

\begin{table*}[tbh!]
  \centering
  \resizebox{16cm}{!}{
  \begin{tabular}{p{6cm}|p{4cm}|p{4cm}|p{4cm}}
  \toprule
{\bf Sample Contexts} & {\bf Meena (base)} & {\bf Cleverbot} & {\bf DialoGPT} \\
\midrule
% 3-turn contexts
\aturn{You must have read a lot of books} \newline \bturn{Oh wow, how do you know? Do I look nerdy?} & \bturn{So how do you know?} & \bturn{Never. said I was.} & \bturn{Oh thank goodness.}  \\
\aturn{Of course, you're not!} & \rates{sensible: 1, specific: 1} & \rates{sensible: 0, specific: 0}  & \rates{sensible: 1, specific: 1} \\
\cdashlinelr{1-4}
\aturn{You know nothing, Jon Snow!} \newline \bturn{You must be a fan of Game of Thrones}  & \bturn{Who's your favorite character?} & \bturn{What do you mean?} & \bturn{You can't. But that's not why you shouldn't know.} \\
\aturn{Haha yea, how can I not?} & \rates{sensible: 1, specific: 1} & \rates{sensible: 0, specific: 0} & \rates{sensible: 0, specific: 0} \\
\cdashlinelr{1-4}
\aturn{What is your favorite island in the world?} \newline \bturn{I would say Fiji} & \bturn{Just a beautiful place} & \bturn{The title is self explanatory.} & \bturn{You can see some great scenery.} \\
\aturn{Interesting, what's nice about it?} & \rates{sensible: 1, specific: 0} & \rates{sensible: 0, specific: 0} & \rates{sensible: 1, specific: 0} \\
\midrule
% 2-turn contexts
\multirow{2}{6cm}{\aturn{You must have read a lot of books} \newline \bturn{Oh wow, how do you know? Do I look nerdy?}} &  \aturn{I know because I've read a lot of books.} & \aturn{Observation.} & \aturn{I know because you look like your mom.} \\
& \rates{sensible: 1, specific: 1} & \rates{sensible: 1, specific: 0} & \rates{sensible: 1, specific: 1} \\
\cdashlinelr{1-4}
\multirow{2}{6cm}{\aturn{You know nothing, Jon Snow!} \newline \bturn{You must be a fan of Game of Thrones}}  & \aturn{Yeah, I'm reading the books at the moment.}  & \aturn{No.} & \aturn{I've never really been interested in it...} \\
& \rates{sensible: 1, specific: 1} & \rates{sensible: 1, specific: 0} & \rates{sensible: 1, specific: 1} \\
\cdashlinelr{1-4}
\multirow{2}{6cm}{\aturn{What is your favorite island in the world?} \newline \bturn{I would say Fiji}} & \aturn{Fiji, yes! I've been there once. It's the most beautiful place I've ever been. It definitely makes me want to move there. I hope you get to visit again soon!} & \aturn{I would have guessed 666.} & \aturn{Fiji is awesome! But I would say Fiji and Oceania are more popular at the moment.} \\
& \rates{sensible: 1, specific: 1} & \rates{sensible: 0, specific: 0}  & \rates{sensible: 0, specific: 0} \\
\midrule
% 1-turn
\multirow{2}{6cm}{\aturn{You must have read a lot of books}} & \bturn{Reading's for nerds} & \bturn{What books have you read.} & \bturn{I read a lot of books but have never read a single book about the history of our planet.} \\
& \rates{sensible: 1, specific: 1} & \rates{sensible: 1, specific: 1} & \rates{sensible: 1, specific: 1} \\
\cdashlinelr{1-4}
\multirow{2}{6cm}{\aturn{You know nothing, Jon Snow!}} & \bturn{Thank you for this. I was hoping I wasn't the only one getting an ASOIAF vibe from this.} & \bturn{Am not jon snow.} & \bturn{The North Remembers...} \\
& \rates{sensible: 1, specific: 1} & \rates{sensible: 1, specific: 0} & \rates{sensible: 1, specific: 1} \\
\cdashlinelr{1-4}
\multirow{2}{6cm}{\aturn{What is your favorite island in the world?}} & \bturn{That's a tough one. I'd have to say Hawaii.} & \bturn{Daniel I like frites.} & \bturn{Probably the one on the north island} \\
& \rates{sensible: 1, specific: 1} & \rates{sensible: 0, specific: 0} & \rates{sensible: 0, specific: 0} \\
\bottomrule
  \end{tabular}
  }
  \caption{{\bf Sample responses from static evaluation} -- Shown are responses of Meena (base), Cleverbot, and DialoGPT on some sample contexts together with their binary labels per category (sensibleness and specificity). Note that the contexts were constructed in advance before we generate all model responses. These contexts are not in the MTB dataset.}
  \label{t:static_analysis}
\end{table*}

\subsection{XiaoIce, Mitsuku, DialoGPT and Cleverbot}
\label{sec:results_other_bots}
Crowd workers labeled 1,173 XiaoIce turns within their original conversation context. Per these labels, XiaoIce scores 31\% interactive SSA which is comprised of 45\% sensibleness and 17\% specificity. We used majority voting of 5 workers per chatbot response. Agreement between workers was 77\% for sensibleness and 81\% for specificity and Krippendorff's alpha was 0.54 for sensibleness and 0.40 for specificity (which indicates fairly strong agreement). For further verification of the results, we also had a group of 4 internal company volunteers that are native Mandarin speakers to label a subset of 25 conversations (~247 chatbot turns). The volunteers did not know the crowd worker results. The volunteer based estimate is 36\% interactive SSA with 53\% sensibleness and 19\% specificity.

Volunteers report that XiaoIce responses display empathy and personality. However, the responses do not always make sense and are often generic. The generic responses exuded a fun personality, but were not necessarily related to the ongoing conversation. As mentioned above, XiaoIce is reported to be optimized for long term engagement \citep{xiaoice}. It is also designed with a multifaceted notion of `humanlikeness' in mind, emphasising interpersonal qualities such as empathy. As we discuss in Section~\ref{sec:discussion}, a broader metric of humanlikeness would be a useful topic for future research.

\citet{see19} report engagingness is not the same as humanness. In that work, they control and optimize certain attributes of response generation. One of the results is that their chatbots achieve near-human-level engagingness, but simultaneously are not very close to human-level humanness. This along with limitations described in Section \ref{sec:xiaoice_mitsuku_eval} may help explain why XiaoIce's sensibleness and specificity scores seem relatively low in our evaluation.

Mitsuku scores 56\% interactive SSA with 72\% sensibleness and 40\% specificity over 899 chatbot turns. Mitsuku has won the Loebner prize 5 times,\footnote{\url{https://en.wikipedia.org/w/index.php?title=Loebner_Prize&oldid=927503336}} however, we learned from the Pandorabots team that the website version we tested with was not the one that competed in the Loebner prize. Optimizing human likeness for the competition might correlate more with our metrics.

Using crowd workers, we executed interactive evaluation of DialoGPT over 300 conversations (2,660 chatbot turns labeled). DialoGPT scores $48\% \pm 3\%$ interactive SSA with $57\% \pm 2\%$ sensibleness and $39\% \pm 4\%$ specificity. It obtained similar results in static evaluation. In its paper, DialoGPT attains performance close to human in a single-turn setting. On the other hand, our human evaluation is multi-turn, which is expected to be more challenging. Additionally, DialoGPT scores poorly on specificity, and our impression from browsing transcripts is that it prefers briefer and more generic responses. This might be because the model is optimized for classic Turing-test evaluation, in which overly chatty responses increase the risk of making a mistake. These results and conjectures come with the caveat, as described above, that we wrote our own decoder for this model since the public DialoGPT codebase does not yet have one.

Cleverbot, unlike Meena and DialoGPT, performs notably better on interactive rather than static evaluation. It scores interactive SSA 56\% and static SSA 44\%. Interactive specificity, 45\%, is especially higher than its static counterpart, 28\%. Upon closer inspection of the data, we hypothesize that: (1) in the interactive setting, Cleverbot has opportunities to steer the conversation towards topics that it is more familiar with; (2) the minimum interactive conversation length of 14 turns makes it possible for a significant portion of these turns to be greetings and goodbyes, which both Cleverbot and Mitsuku are consistent in appropriately responding to. Furthermore, the interactive SSA scores for Mitsuku and Cleverbot are the same, 56\% when averaging sensibleness and specificity before rounding. Mitsuku scores higher sensibleness (72\% versus 68\%), but lower specificity (40\% versus 45\%). It seems that relative to Mitsuku, Cleverbot replies more often in ways that are borderline nonsensical and lack consistent personality. Finally, we remark that the standard deviation of the Cleverbot interactive SSA is $\pm1\%$ across two interactive evaluation sessions.\footnote{Due to technical issues when calling the Cleverbot API we only collected 195 interactive conversations (1,751 chatbot turns labeled) instead of the 300 conversations which we collected for DialoGPT.}

\subsection{Sample Responses: \meenabase{}, Cleverbot, and DialoGPT}
To understand how Meena qualitatively compares to other models, we show in Table~\ref{t:static_analysis} sample responses from \meenabase{}, Cleverbot, and DialoGPT under the same set of contexts (which were constructed before we generate all model responses). For 1- and 2-turn contexts,  responses from Meena base are all sensible and specific.
In addition, \meenabase{} generates rich and interesting responses, e.g., the mention of \textit{``ASOIAF vibe''} to refer to ``A Song of Ice and Fire'' in the famous Game of Thrones series or the remark about Fiji island being \textit{``the most beautiful place I've ever been''}.

In contrast, Cleverbot can generate sensible responses for some contexts, but they are not always specific, e.g., Cleverbot replied with \textit{``Observation''} and \textit{``No''}. DialoGPT is more specific and can also generate interesting responses, e.g., \textit{``The North Remembers ...'''}. However, it does not make sense at times, e.g., in-turn contradiction in this response \textit{``Fiji is awesome! But I would say Fiji and Oceania are more popular ...''} or vague answer \textit{``Probably the one on the north island''}.

When it comes to longer (3-turn) contexts in Table~\ref{t:static_analysis}, \meenabase{} continues to generate high-quality responses, whereas none of Cleverbot's responses are sensible.
DialoGPT is more sensible and specific than Cleverbot, but less so than \meenabase{}.
